How many geodesics join two points on a contact sub-Riemannian manifold?

We investigate the number of geodesics between two points $p$ and $q$ on a contact sub-Riemannian manifold M. We show that the count of geodesics on $M$ is controlled by the count on its nilpotent approximation at $p$ (a contact Carnot group). For contact Carnot groups we make the count explicit in exponential coordinates $(x,z) \in \mathbb{R}^{2n} \times \mathbb{R}$ centered at $p$. In this case we prove that for the generic $q$ the number of geodesics $\nu(q)$ between $p$ and $q=(x,z)$ satisfies: \[ C_1\frac{|z|}{\|x\|^2} + R_1 \leq \nu(q) \leq C_2\frac{|z|}{\|x\|^2} + R_2\] for some constants $C_1,C_2$ and $R_1,R_2$. We recover exact values for Heisenberg groups, where $C_1=C_2 = \frac{8}{\pi}$. Removing the genericity condition for $q$, geodesics might appear in families and we prove a similar statement for their topology. We study these families, and in particular we focus on the unexpected appearance of isometrically non-equivalent geodesics: families on which the action of isometries is not transitive. We apply the previous study to contact sub-Riemannian manifolds: we prove that for any given point $p \in M$ there is a sequence of points $p_n$ such that $p_n \to p$ and that the number of geodesics between $p$ and $p_n$ grows unbounded (moreover these geodesics have the property of being contained in a small neighborhood of $p$).

==> global.tex <==
%!TEX root = enumerative.tex
\section{A global count}
In this section we discuss the existence of infinitely many ``non-local'' geodesics.
The result still holds true in much generality, but for our purpose we state them only for contact sub-Riemannian manifolds.

We recall the following theorem, due to J-P. Serre.

\begin{theorem}[Serre]Let $M$ be a connected, complete Riemannian manifold such that the homology group $H_k(M. \Z)$ is non-zero for at least one integer $k.$ Then given two distinct points $p_0$ and $p$ on $M$, there exist infinitely many geodesics joining them.
\end{theorem}

We will generalize this theorem to the following one. The first part of the proof is essentially identical to Serre's one; the new ingredients are the fact that the \emph{horizontal} path space is homotopy equivalent to the standard one (the equivalence being given by the inclusion) and the fact that there are no abnormal geodesic between two distinct points on a contact sub-Riemannian manifold.

\begin{theorem}Let $M$ be a connected, complete contact sub-Riemannian manifold such that the homology group $H_k(M. \Z)$ is non-zero for at least one integer $k.$ Given two distinct points $p_0$ and $p$ on $M$ and an open contractible set $U$ containing both $p_0$ and $p$, 
 there exist infinitely many sub-Riemannian geodesics joining them not entirely contained in $U$.
\end{theorem}
Thus in particular, as long as $M$ has non-trivial homology, not only when $p_0$ and $p$ approach there are more and more geodesics all contained in a privileged coordinates chart neighborhood, but also there are infinitely many escaping out of this neighborhood.
\begin{proof}As we said we repeat verbatim Serre's proof, modifying it only when necessary. Let us start by considering the universal cover $\overline{M}$ of $M$:
\be q:\overline{M}\to M.\ee
Then if $\alpha$ is the contact one-form of $M$, $q^*\alpha$ is a contact form on 
$\overline{M}$ and the sub-Riemannian structure on $\overline\Delta=\ker q^*\alpha$ is pulled back as well by simply defining $ \langle v_1, v_2\rangle=\langle dq v_1, dq v_2\rangle$  for all $ v_1, v_2\in \overline\Delta.$

It is easy to check that a sub-Riemannian geodesic $\overline \gamma$ projects via $q$ to a sub-Riemannian geodesic $q\overline{\gamma}$; in partcular if we pick $\overline p_0 $ such that $q(\overline p_0)=p_0$, the set of geodesics joining $p_0$ and $p$ is in one-to-one correspondence with the set of geodesics joining $\overline{p}_0$ and a point in $q^{-1}(p).$

We distinguish two cases: the case when $\pi_1(M)$ is infinite and the case when is finite. 

In the case it is infinite for every $0\neq [\gamma]\in \pi_1(M, p_0)$ let $\overline\gamma$ a path between $\overline p_0$ and another point in $q^{-1}(p_0)$ lifting $\gamma$. Since $\overline M$ is contact, the bracket generating condition is satisfied and we can choose $\overline{\gamma}$ to be a minimal geodesic. In this case $\gamma$ cannot be all contained in $U$ otherwise $[\gamma]=0$. This yields infinitely many geodesics not contained in $U$.

In the case $\pi_1(M)$ is finite, then there exists $k>0$ such that $H_k(\overline{M}, \Z)\neq 0$ (see \cite[Exposee XII]{Cartan}). Following \cite[Proposition 3, Section 3]{Serre} we obtain the existence of a field $\mathbb{K}$ and an integer $k>0$ such that $H_k(\overline{M}, \mathbb{K})\neq 0$. This implies that, given $\overline{p}\in \overline{M}$,  there are infinitely many $i$ such that $H_i(\Omega_{\overline{p}}^{\textrm{st}}, \mathbb{K})$ is different from zero (here $\Omega_{\overline{p}}^{\textrm{st}}$ is the ``standard'' space of paths between $\overline{p}_0$ and $\overline{p}$, with no horizontal restrictions). 

At this point we use the fact that in the contact case $\Omega_{\overline{p}}\hookrightarrow \Omega_{\overline{p}}^{\textrm{st}}$ is indeed a homotopy equivalence \cite{Ge, Sarychev}, and thus: 
\be H_k(\Omega_{\overline{p}}, \mathbb{K})\neq 0\quad \textrm{for infinitely many integers $k$}.\ee
We notice now that, as long as $\overline p\neq \overline p_0$, the space $\Omega_{\overline{p}}$ is a (smooth) Hilbert manifold: in fact the only critical point of the endpoint map $F:\Omega\to \overline{M}$ is the constant curve $\gamma(t)\equiv \overline{p}_0$ (see \cite{Agrachevcontact}).
\end{proof}



